AGaLiTe: Approximate Gated Linear Transformers for Online Reinforcement Learning

In this paper we investigate transformer architectures designed for partially observable online reinforcement learning. The self-attention mechanism in the transformer architecture is capable of capturing long-range dependencies and it is the main reason behind its effectiveness in processing sequential data. Nevertheless, despite their success, transformers have two significant drawbacks that still limit their applicability in online reinforcement learning: (1) in order to remember all past information, the self-attention mechanism requires access to the whole history to be provided as context. (2) The inference cost in transformers is expensive. In this paper, we introduce recurrent alternatives to the transformer self-attention mechanism that offer context-independent inference cost, leverage long-range dependencies effectively, and performs well in online reinforcement learning task. We quantify the impact of the different components of our architecture in a diagnostic environment and assess performance gains in 2D and 3D pixel-based partially-observable environments (e.g. T-Maze, Mystery Path, Craftax, and Memory Maze). Compared with a state-of-the-art architecture, GTrXL, inference in our approach is at least 40% cheaper while reducing memory use more than 50%. Our approach either performs similarly or better than GTrXL, improving more than 37% upon GTrXL performance in harder tasks.

==> fresh_experiments.tex <==
To elaborate on the computational efficiency of our approach, we can compare the exact number operations and the space required when using typical hyperparameter values. As an estimate of the number of operations, we calculate the total number of floating point operations required to process a single element in a streaming sequence. To estimate the space required, we calculate the total number of floating point numbers required to store the recurrent state. For GTrXL self-attention we consider the hyperparameter values from \cite{parisotto2020stabilizing}, that is $M=512$, $d=256$ and $d_h=64$. For ReLiT, we consider $d=256$, $d_h=64$, and $\eta=4$. The goal is to match the hyperparameters of the GTrXL architecture as closely as possible and chose typical values for the novel hyperparameters. We chose $\eta=4$ as we found it to work reasonably well in our experiments. ReLiT self-attention is roughly 110.95 times faster than GTrXL self-attention and uses 7.87 times less space. This improvement in time and space is only possible because the complexity of ReLiT self-attention does not depend on the context length.
